Don't Just Chase "Highlighted Tokens" in MLLMs: Revisiting Visual Holistic Context Retention

Despite their powerful capabilities, Multimodal Large Language Models (MLLMs) suffer from considerable computational overhead due to their reliance on massive visual tokens. Recent studies have explored token pruning to alleviate this problem, which typically uses text-vision cross-attention or [\texttt{CLS}] attention to assess and discard redundant visual tokens. In this work, we identify a critical limitation of such attention-first pruning approaches, i.e., they tend to preserve semantically similar tokens, resulting in pronounced performance drops under high pruning ratios. To this end, we propose {HoloV}, a simple yet effective, plug-and-play visual token pruning framework for efficient inference. Distinct from previous attention-first schemes, HoloV rethinks token retention from a holistic perspective. By adaptively distributing the pruning budget across different spatial crops, HoloV ensures that the retained tokens capture the global visual context rather than isolated salient features. This strategy minimizes representational collapse and maintains task-relevant information even under aggressive pruning. Experimental results demonstrate that our HoloV achieves superior performance across various tasks, MLLM architectures, and pruning ratios compared to SOTA methods. For instance, LLaVA1.5 equipped with HoloV preserves 95.8\% of the original performance after pruning 88.9\% of visual tokens, achieving superior efficiency-accuracy trade-offs.

==> tables/frame_compared.tex <==
\begin{table}[!tb]
\centering
\caption{Comprehensive comparisons between the proposed MemVR and existing approaches are presented. MemVR introduces a low-latency \textit{look-twice} decoding mechanism.
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccc}
        \toprule
        {Methods}  & {{\begin{tabular}[c]{@{}c@{}}General
 \\ Performance \end{tabular}}} & {\begin{tabular}[c]{@{}c@{}}Computational \\Complexity \end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Pruning \\Strategies\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Training  \\-free \end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Attention  \\Categories \end{tabular}} \\
        \midrule
        ToMe \cite{bolya2023token}   & xx     & Low & Low     & Low & Contrastive \\
        
        FastV \cite{chen2024image}  & Medium    & Low & High  & Low        & Att-intervention \\
        
        HiRED \cite{arif2024hired} & Location and Features  & Low & High & Low          & Att-intervention \\ 
        
        LLaVA-PruMerge \cite{shang2024llava} & Clustering-based  & Low & High & Low          & Att-intervention   \\ 
        
        SparseVLM \cite{zhang2024sparsevlm}  & Medium & Low & Medium          & Low        & Contrastive     \\     

        
        FasterVLM \cite{zhang2024cls}  & Medium  & Low & Ultrahigh          & Low      & Contrastive   \\
        
        PDrop \cite{xing2024pyramiddrop}  & Medium  & Low & Ultrahigh          & Low      & Contrastive    \\
        
        FiCoCo-V \cite{han2024rethinking}  & Medium  & Low & Ultrahigh          & Low      & Contrastive    \\
        
        MustDrop \cite{liu2024multi}  & Medium  & Low & Ultrahigh          & Low      & Contrastive   \\
        
        WiCo \cite{Li2025window}   & Medium  & Low & Ultrahigh          & Low      & Contrastive   \\
        
        ALTP \cite{bai2025local}  & Medium  & Low & Ultrahigh          & Low      & Contrastive   \\
        
        \cellcolor{lightgray}HoloV (ours)  & \cellcolor{lightgray}High   & \cellcolor{lightgray}Low & \cellcolor{lightgray}Low & \cellcolor{lightgray}Low   & \cellcolor{lightgray}\texttt{[CLS]} Attention \\
        \bottomrule
\end{tabular}
}\label{tab2:comparison} \vspace{-0.25em}
\end{table}

==> tables/table4.tex <==

\begin{table}[t]
    \vspace{-0.75em}
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \footnotesize
    \caption{Comparisons of various methods on image understanding. Results are shown for different pruning ratios, highlighting the accuracy and average performance of each method.}
    \vspace{0.25em}
    \label{tab:main}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l | *{9}{>{\centering\arraybackslash}p{0.92cm}} |>{\centering\arraybackslash}p{1.15cm}}
        \toprule[1.25pt]
        \textbf{\;Methods} & \textbf{GQA} & \textbf{MMB} & \textbf{MMB}$_{\text{CN}}$ & \textbf{MME} & \textbf{POPE} & \textbf{SQA} & \textbf{VQA}$_{\text{V2}}$ & \textbf{VQA}$_{\text{Text}}$ & \textbf{VizWiz}  & \makecell[c]{\textbf{Average}}\\
        \midrule
        
        % LLaVA-1.5-7B & \multicolumn{11}{c}{ \ $(100\%)$}\\
        \textcolor{gray}{Upper Bound, 576 Tokens} & \textcolor{gray}{61.9} & \textcolor{gray}{64.7} & \textcolor{gray}{58.1} & \textcolor{gray}{1862} & \textcolor{gray}{85.9} & \textcolor{gray}{69.5} & \textcolor{gray}{78.4} & \textcolor{gray}{58.2} & \textcolor{gray}{50.0} & \multirow{1}*{\textcolor{gray}{100\%}} \\
        % ~ & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & ~ \\
        \midrule

        \rowcolor{mygray}
        LLaVA-1.5 \textcolor{gray}{7B} & \multicolumn{10}{c}{\textit{Retain 192 Tokens} \ $\fg{(\downarrow 66.7\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 54.3 & 60.5 & - & 1563 & 72.4 & 65.2 & 68.0 & 52.1 & - & \multirow{1}*{88.5\%} \\
        % ~ & 87.7\% & 93.5\% & 83.9\% & 84.3\% & 93.8\% & 86.6\% & 89.5\% & ~ \\
        % \hline
        FastV \texttt{\scriptsize{(ECCV24)}} & 52.7 & 61.2 & 57.0 & 1612 & 64.8 & 67.3 & 67.1 & 52.5 & 50.8  & \multirow{1}*{90.5\%} \\
        % ~ & 85.1\% & 94.6\% & 86.6\% & 75.4\% & 96.8\% & 85.5\% & 90.2\% & ~ \\
        % \hline
        LLaVA-PruMerge \texttt{\scriptsize{(ICCV25)}}\;\; & 54.3 & 59.6 & 52.9 & 1632 & 71.3 & 67.9 & 70.6 & 54.3 & 50.1  & 91.4\% \\
        PDrop \texttt{\scriptsize{(CVPR25)}} & 57.1 & 63.2 & 56.8 & 1766 & 82.3 & 68.8 & 75.1 & 56.1 & 51.1  & 96.7\% \\
        FiCoCo-V \texttt{\scriptsize{(2025.03)}} & 58.5 & 62.3 & 55.3 & 1732 & 82.5 & 67.8 & 74.4 & 55.7 & 51.0  & 96.1\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 58.2 & 62.3 & 55.8 & 1787 & 82.6 & 69.2 & 76.0 & 56.5 & \textcolor{MidnightBlue}{51.4}  & 97.2\% \\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 58.7 & 62.8 & 54.7 & 1737 & 82.8 & 68.4 & 74.9 & 47.4 & 50.1  & 94.6\%     \\
        SparseVLM \texttt{\scriptsize{(2025.2)}} & 57.6 & 62.5 & 53.7 & 1721 & {83.6} & 69.1 & 75.6 & 56.1 & 50.5  & 96.1\% \\
        % \rowcolor{mygreen1}
        % HoloV \scriptsize{(Ours)} & {60.0} & {63.6} & {57.0} & {1856} & 82.8 & {69.8} & {76.7} & {57.4} & 51.2 & {296} & {98.8\%} \\
        \rowcolor{mygreen2}
        HoloV$^\dagger$ \scriptsize{(Ours)} & \textcolor{MidnightBlue}{59.0} & \textcolor{MidnightBlue}{65.4} & \textcolor{MidnightBlue}{58.0} & \textcolor{MidnightBlue}{1820} & \textcolor{MidnightBlue}{85.6} & \textcolor{MidnightBlue}{69.8} & \textcolor{MidnightBlue}{76.7} & \textcolor{MidnightBlue}{57.4} & 50.9  & \textcolor{MidnightBlue}{99.2\%} \\
        \midrule

        \rowcolor{mygray}
        LLaVA-1.5 \textcolor{gray}{7B} & \multicolumn{10}{c}{\textit{Retain 128 Tokens} \ $\fg{(\downarrow 77.8\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 52.4 & 53.3 & - & 1343 & 62.8 & 59.6 & 63.0 & 49.1 & - & \multirow{1}*{80.4\%} \\
        % ~ & 84.7\% & 82.4\% & 72.1\% & 73.1\% & 85.8\% & 80.2\% & 84.4\% & ~ \\
        % \hline
        FastV \texttt{\scriptsize{(ECCV24)}} & 49.6 & 56.1 & 56.4 & 1490 & 59.6 & 60.2 & 61.8 & 50.6 & 51.3  & \multirow{1}*{85.4\%}\\
        % ~ & 80.1\% & 86.7\% & 80.0\% & 69.4\% & 86.6\% & 78.7\% & 86.9\% & ~\\
        % \hline
        LLaVA-PruMerge \texttt{\scriptsize{(ICCV25)}} & 53.3 & 58.1 & 51.7 & 1554 & 67.2 & 67.1 & 68.8 & 54.3 & 50.3  & 89.4\%  \\
        % ~ & 90.5\% & 92.7\% & 91.1\% & 93.7\% & 96.5\% & 94.0\% & 94.3\% & $\fr{\uparrow(11.4\%)}$ \\
        PDrop \texttt{\scriptsize{(CVPR25)}} & 56.0 & 61.1 & \textcolor{MidnightBlue}{56.6} & 1644 & {82.3} & 68.3 & 72.9 & 55.1 & 51.0 & 94.9\% \\
        FiCoCo-V \texttt{\scriptsize{(2025.03)}} & 57.6 & 61.1 & 54.3 & 1711 & 82.2 & 68.3 & 73.1 & 55.6 & 49.4  & 94.9\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 56.9 & 61.1 & 55.2 & 1745 & 78.7 & 68.5 & 74.6 & 56.3 & \textcolor{MidnightBlue}{52.1}  & 95.7\% \\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 57.2 & 61.5 & 53.6 & 1710 & 79.8 & 68.1 & 73.4 & 46.1 & 51.3  & 93.1\% \\
        SparseVLM
         \texttt{\scriptsize{(2025.2)}} & 56.0 & 60.0 & 51.1 & 1696 & 80.5 & 67.1 & 73.8 & 54.9 & 51.4 & 93.8\% \\
        % \rowcolor{mygreen1} HoloV \scriptsize{(Ours)} & {58.7} & {63.2} & {57.5} & {1840} & 80.1 & {69.1} & {75.9} & {56.4} & 51.7 & {296} & {98.0\%} \\
        \rowcolor{mygreen2} HoloV$^\dagger$ \scriptsize{(Ours)} & \textcolor{MidnightBlue}{57.7} & \textcolor{MidnightBlue}{63.9} & {56.5} & \textcolor{MidnightBlue}{1802} & \textcolor{MidnightBlue}{84.0} & \textcolor{MidnightBlue}{69.8} & \textcolor{MidnightBlue}{75.5} & \textcolor{MidnightBlue}{56.8} & 51.5  & \textcolor{MidnightBlue}{98.0\%} \\
        \midrule

        \rowcolor{mygray}
        LLaVA-1.5 \textcolor{gray}{7B} & \multicolumn{10}{c}{\textit{Retain 64 Tokens} \ $\fg{(\downarrow 88.9\%)}$}\\
        ToMe \texttt{\scriptsize{(ICLR23)}} & 48.6 & 43.7 & - & 1138 & 52.5 & 50.0 & 57.1 & 45.3 & -  & \multirow{1}*{70.1\%}\\
        % ~ & 78.5\% & 67.5\% & 61.1\% & 61.1\% & 71.9\% & 72.7\% & 77.8\% & ~\\
        % \hline
        FastV \texttt{\scriptsize{(ECCV24)}} & 46.1 & 48.0 & 52.7 & 1256 & 48.0 & 51.1 & 55.0 & 47.8 & 50.8  & 76.7\% \\
        % ~ & 74.5\% & 74.2\% & 67.5\% & 55.9\% & 73.5\% & 70.1\% & 82.1\% & ~\\
        % \hline
        LLaVA-PruMerge \texttt{\scriptsize{(ICCV25)}} & 51.9 & 55.3 & 49.1 & 1549 & 65.3 & 68.1 & 67.4 & 54.0 & 50.1 & 87.7\% \\
        % ~ & 85.1\% & 86.9\% & 80.8\% & 87.4\% & 89.4\% & 86.9\% & 89.0\% & $\fr{\uparrow(14.8\%)}$  \\
        PDrop \texttt{\scriptsize{(CVPR25)}} & 41.9 & 33.3 & 50.5 & 1092 & 55.9 & 68.6 & 69.2 & 45.9 & 50.7 & 77.5\% \\
        FiCoCo-V \texttt{\scriptsize{(2025.03)}} & 52.4 & 60.3 & 53.0 & 1591 & {76.0} & 68.1 & 71.3 & 53.6 & 49.8  & 91.5\% \\
        MustDrop \texttt{\scriptsize{(2024.11)}} & 53.1 & 60.0 & 53.1 & 1612 & 68.0 & 63.4 & 69.3 & 54.2 & 51.2  & 90.1\%    \\
        HiRED \texttt{\scriptsize{(AAAI25)}} & 54.6 & 60.2 & 51.4 & 1599 & 73.6 & 68.2 & 69.7 & 44.2 & 50.2  & 89.4\% \\
        SparseVLM \texttt{\scriptsize{(2025.2)}} & 52.7 & 56.2 & 46.1 & 1505 & 75.1 & 62.2 & 68.2 & 51.8 & 50.1  & 87.3\% \\
        % \rowcolor{mygreen1} HoloV \scriptsize{(Ours)} & {55.9} & {60.6} & {53.2} & {1765} & 73.9 & {69.8} & {72.4} & {54.4} & {51.6} & {270} & {93.7\%} \\
        \rowcolor{mygreen2} HoloV$^\dagger$ \scriptsize{(Ours)} & \textcolor{MidnightBlue}{55.3} & \textcolor{MidnightBlue}{63.3} & \textcolor{MidnightBlue}{55.1} & \textcolor{MidnightBlue}{1715} & \textcolor{MidnightBlue}{80.3} & \textcolor{MidnightBlue}{69.5} & \textcolor{MidnightBlue}{72.8} & \textcolor{MidnightBlue}{55.4} & \textcolor{MidnightBlue}{52.8} & \textcolor{MidnightBlue}{95.7\%} \\
        \bottomrule[1.25pt]
	\end{tabular}
    }
\end{table}


